Few-Shot Classification with Contrastive Learning

A two-stage training paradigm consisting of sequential pre-training and meta-training stages has been widely used in current few-shot learning (FSL) research. Many of these methods use self-supervised learning and contrastive learning to achieve new state-of-the-art results. However, the potential of contrastive learning in both stages of FSL training paradigm is still not fully exploited. In this paper, we propose a novel contrastive learning-based framework that seamlessly integrates contrastive learning into both stages to improve the performance of few-shot classification. In the pre-training stage, we propose a self-supervised contrastive loss in the forms of feature vector vs. feature map and feature map vs. feature map, which uses global and local information to learn good initial representations. In the meta-training stage, we propose a cross-view episodic training mechanism to perform the nearest centroid classification on two different views of the same episode and adopt a distance-scaled contrastive loss based on them. These two strategies force the model to overcome the bias between views and promote the transferability of representations. Extensive experiments on three benchmark datasets demonstrate that our method achieves competitive results.

==> SM_submission.tex <==
% updated April 2002 by Antje Endemann
% Based on CVPR 07 and LNCS, with modifications by DAF, AZ and elle, 2008 and AA, 2010, and CC, 2011; TT, 2014; AAS, 2016; AAS, 2020; TH, 2022

% \documentclass[runningheads]{llncs}
% \usepackage{graphicx}
% DO NOT USE \usepackage{times}, it will be removed by typesetters
%\usepackage{times}

% \usepackage{tikz}
% \usepackage{comment}
% \usepackage{amsmath,amssymb} % define this before the line numbering.
% \usepackage{color}
% \usepackage{orcidlink}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
% \usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.


% INITIAL SUBMISSION - The following two lines are NOT commented
% CAMERA READY - Comment OUT the following two lines
% \usepackage{ruler}
% \usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{subcaption}
% \usepackage{hyperref}
% \hypersetup{
%     bookmarks=true,
% 	colorlinks=true,
% 	linkcolor=blue,
% 	filecolor=blue,
%     urlcolor=blue,
% 	citecolor=blue,
% }

% \begin{document}
% \renewcommand\thelinenumber{\color[rgb]{0.2,0.5,0.8}\normalfont\sffamily\scriptsize\arabic{linenumber}\color[rgb]{0,0,0}}
% \renewcommand\makeLineNumber {\hss\thelinenumber\ \hspace{6mm} \rlap{\hskip\textwidth\ \hspace{6.5mm}\thelinenumber}}
% \linenumbers
% \pagestyle{headings}
% \mainmatter
% \def\ECCVSubNumber{4929}  % Insert your submission number here

% \title{Few-Shot Classification with Contrastive Learning \\ Supplementary Material}

% INITIAL SUBMISSION
%******************

% CAMERA READY SUBMISSION
% \begin{comment}
% \titlerunning{Few-Shot Classification with Contrastive Learning}
% If the paper title is too long for the running head, you can set
% an abbreviated paper title here
%
% \author{Zhanyuan Yang\inst{1} \and
% Jinghua Wang\inst{2} \and
% Yingying Zhu\thanks{Corresponding author.}\inst{1}}
% %
% \authorrunning{Zy. Yang et al.}
% % First names are abbreviated in the running head.
% % If there are more than two authors, 'et al.' is used.
% %
% \institute{College of Computer Science and Software Engineering, Shenzhen University, Shenzhen, China\\
% % \and
% \email{yangzhanyuan2019@email.szu.edu.cn, zhuyy@szu.edu.cn}
% % \\
% \and
% School of Computer Science and Technology, Harbin Institute of Technology (Shenzhen), Shenzhen, China\\
% \email{wangjinghua@hit.edu.cn}}
% \end{comment}
%******************
% \maketitle


\section{Additional Ablation Study}
We conduct ablation studies in the pre-training stage on the miniImageNet.
Here, except for the model trained with only $L_{CE}$ (see the first line in \tablename~\ref{tab:pretrain_loss}), we adopt cross-view episodic training (CVET) mechanism and distance-scaled contrastive loss in the meta-training stage for all experiments in \tablename~\ref{tab:pretrain_loss} and \tablename~\ref{tab:pretrain_local}.

\vspace{-15pt}

\begin{table*}[!ht]
\centering
\caption{Ablation experiments in the pre-training stage on miniImageNet.}
\renewcommand\arraystretch{1.2}
% \resizebox{.60\columnwidth}{!}{
\begin{tabular}{c|ccc|c|c}
\hline
$L_{CE}$                & $L_{global}^{ss}$ & $L_{local}^{ss}$ & $L_{global}^{s}$ & \textbf{1-shot}       & \textbf{5-shot}        \\ \hline
$\surd$ &                                       &                                      &                                      & 66.58 ± 0.46          & 81.92 ± 0.31          \\
$\surd$ & $\surd$                  &                                      &                                      & 68.53 ± 0.46 & 83.86 ± 0.29 \\
$\surd$ &                                       & $\surd$                 &                                      & 69.33 ± 0.46 & 84.02 ± 0.30 \\
$\surd$ &                                       &                                      & $\surd$                 & 67.88 ± 0.45 & 83.37 ± 0.29 \\
$\surd$ & $\surd$                  & $\surd$                 &                                      & 69.03 ± 0.46 & 83.87 ± 0.30 \\
$\surd$ & $\surd$                  &                                      & $\surd$                 & 68.68 ± 0.46 & 84.17 ± 0.29 \\
$\surd$ &                                       & $\surd$                 & $\surd$                 & 69.72 ± 0.45 & 84.49 ± 0.29 \\
$\surd$ & $\surd$                  & $\surd$                 & $\surd$                 & 70.19 ± 0.46 & 84.66 ± 0.29 \\ \hline
\end{tabular}
% }
\label{tab:pretrain_loss}
\end{table*}

\vspace{-25pt}

\begin{table*}[!ht]
\centering
\caption{Effectiveness of vector-map and map-map modules on miniImageNet.}
\renewcommand\arraystretch{1.5}
% \resizebox{.70\columnwidth}{!}{
\begin{tabular}{c|cc|c|c}
\hline
$L_{CE}+L_{global}^{ss}+L_{global}^{s}$ & $L_{vec-map}^{ss}$ & $L_{map-map}^{ss}$ & \textbf{1-shot} & \textbf{5-shot} \\\hline
$\surd$     &            &                &  68.68 ± 0.46   &  84.17 ± 0.29   \\
$\surd$     & $\surd$           &                & 69.29 ± 0.46    & 84.23 ± 0.29    \\
$\surd$     &                & $\surd$           & 68.81 ± 0.46    & 84.25 ± 0.29    \\
$\surd$     &  $\surd$              & $\surd$           & 70.19 ± 0.46    & 84.66 ± 0.29    \\ \hline
\end{tabular}
% }
\label{tab:pretrain_local}
\end{table*}

As shown in \tablename~\ref{tab:pretrain_loss}, compared to training with $L_{CE}$ alone, each contrastive loss used in the pre-training stage plays an important role, with $L_{local}^{ss}$ contributing the most.
The results from the methods introducing $L_{local}^{ss}$ indicate that contrastive learning based on extra local information can learn more generalizable representations.
Meanwhile, we can observe that the results obtained by training with supervision only are much lower than the results obtained by using both supervision and self-supervision.
The results in \tablename~\ref{tab:pretrain_loss} validate the effectiveness of our proposed contrastive losses, and we obtain the best results when employing all proposed contrastive losses in the pre-training stage.

Based on $L_{CE}$ and the other two contrastive losses using global information, we verify the effectiveness of vector-map and map-map modules by conducting experiments on them separately, as shown in \tablename~\ref{tab:pretrain_local}.
Compared to using only global information, contrastive learning that leverages local information either in the form of vector-map or map-map can improve the transferability of the representations.
The best results are achieved when both forms work together.


\newpage


\section{Experiments on Hyperparameters in the Pre-training}
We investigate the effect of hyperparameters in the pre-training stage on classification performance.
%
Note that we use the inverse temperature parameters in our implementation.
To make it easy to understand, we draw the graph according to the inverse temperature parameters.
That is, the horizontal axis of \figurename~\ref{fig:supp_pretrain_robust_a} actually represents the inverse of $\tau_{1,2,3,4}$.
%
As shown in \figurename~\ref{fig:supp_pretrain_robust},
we empirically find that the best results can be achieved by setting the four temperature parameters $\tau_{1,2,3,4}$ to 0.1 and the three balance scalars $\alpha_{1,2,3}$ to 1.0 at the same time.
%
The results indicate that our pre-training approach is less sensitive to the two kinds of hyperparameters (within a certain range), which means it is robust.
Thus it is effortless to apply our approach to other methods.

\begin{figure}[!ht]
\centering
	\begin{minipage}[t]{0.49\columnwidth}
		\includegraphics[width=\linewidth]{fix_alpha.pdf}
        \subcaption{Fix $\alpha_{1,2,3}=1.0$}
        \label{fig:supp_pretrain_robust_a}
	\end{minipage}
	\begin{minipage}[t]{0.49\columnwidth}
		\includegraphics[width=\linewidth]{fix_tau.pdf}
        \subcaption{Fix $\tau_{1,2,3,4}=0.1$}
        \label{fig:supp_pretrain_robust_b}
	\end{minipage}
\caption{Effect of hyperparameters $\tau_{1,2,3,4}$ and $\alpha_{1,2,3}$ on miniImageNet.}
\label{fig:supp_pretrain_robust}
\end{figure}



\newpage

\section{Quantitative Analysis of Model Parameters}
In the case of using the same backbone network, we compare the number of parameters of our proposed method with the two-stage methods ProtoNet~\cite{ProtoNet} and FEAT~\cite{FEAT}.
%
The results are shown in \tablename~\ref{tab:model_params}.
%
In the pre-training stage, the number of parameters of our method is 1.9M more than ProtoNet and baseline (FEAT)
due to the introduction of projection heads and a fully connected layer for our contrastive losses.
%
In the meta-training stage, a single projection head used in distance-scaled contrastive loss results in 0.4M more parameters for our method than baseline.
%
Furthermore, during meta-testing, the number of parameters of our method is the same as in baseline.
%
Therefore, the small number of additional parameters we introduce in the pre-training and meta-training stages is acceptable considering the improved classification performance of our method.

\begin{table}[!ht]
\centering
\caption{Comparison of the number of parameters for several methods.}
\renewcommand\arraystretch{1.2}
% \resizebox{.70\columnwidth}{!}{
\begin{tabular}{l|l|cl|cl}
\hline
Stage                          & Method   & \multicolumn{2}{c|}{Backbone}                   & \multicolumn{2}{c}{\# params} \\ \hline
\multirow{3}{*}{Pre-training}  & ProtoNet~\cite{ProtoNet} & \multicolumn{2}{c|}{\multirow{9}{*}{ResNet-12}} & \multicolumn{2}{c}{12.5M}     \\
                               & FEAT~\cite{FEAT}     & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{12.5M}     \\
                               & Ours     & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{14.4M}     \\ \cline{1-2} \cline{5-6} 
\multirow{3}{*}{Meta-training} & ProtoNet~\cite{ProtoNet} & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{12.4M}     \\
                               & FEAT~\cite{FEAT}     & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{14.1M}     \\
                               & Ours     & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{14.5M}     \\ \cline{1-2} \cline{5-6} 
\multirow{3}{*}{Meta-testing}  & ProtoNet~\cite{ProtoNet} & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{12.4M}     \\
                               & FEAT~\cite{FEAT}     & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{14.1M}     \\
                               & Ours     & \multicolumn{2}{c|}{}                           & \multicolumn{2}{c}{14.1M}     \\ \hline
\end{tabular}
% }
\label{tab:model_params}
\end{table}



\newpage

\section{Qualitative Ablation Study}

In this section, we give qualitative analysis to verify the effectiveness of each component proposed in our method.
%
The classification results of our components are shown in \figurename~\ref{fig:supp_ncm_results},
%
Thanks to the successive use of each component, the model can better adapt to novel tasks with more pictures in which the background is dominant.
%
Moreover, the accurate recognition of small objects reflects that our framework enables the representations to learn meta-knowledge that is useful for few-shot classification.
%
Therefore, it can be considered that each of our proposed components is effective.

\begin{figure}[!ht]
\centering
	\begin{minipage}[t]{0.49\columnwidth}
		\includegraphics[width=\linewidth]{ncm_baseline.pdf}
        \subcaption{baseline}
        \label{fig:supp_ncm_baseline}
	\end{minipage}
	\begin{minipage}[t]{0.49\columnwidth}
		\includegraphics[width=\linewidth]{ncm_baseline+CL.pdf}
        \subcaption{baseline+CL}
        \label{fig:supp_ncm_baseline+CL}
	\end{minipage}
    \\
	\begin{minipage}[t]{0.49\columnwidth}
		\includegraphics[width=\linewidth]{ncm_baseline+CL+CVET.pdf}
        \subcaption{baseline+CL+CVET}
        \label{fig:supp_ncm_baseline+CL+CVET}
	\end{minipage}
	\begin{minipage}[t]{0.49\columnwidth}
		\includegraphics[width=\linewidth]{ncm_ours.pdf}
        \subcaption{Ours}
        \label{fig:supp_ncm_ours}
	\end{minipage}
\caption{5-way 1-shot classification results on miniImageNet. The green box indicates the correct classification result, while the red box indicates the incorrect result.}
\label{fig:supp_ncm_results}
\end{figure}


\newpage

\section{Visualization and Quantitative Analysis of Feature Embeddings}
In this section, we present the complete visualization results of Sect.~4.4 in the paper.
The results from \figurename~\ref{fig:supp_visual_experiment} illustrate that our proposed framework generates more transferable and discriminative representations on novel classes.

\vspace{-10pt}

\begin{figure}[!h]
    \centering
    \begin{minipage}[t]{0.32\columnwidth}
		\centering
        \includegraphics[width=1\linewidth]{ProtoNet.pdf}
        \subcaption{ProtoNet}
		\label{fig:supp_visual_protonet}
	\end{minipage}
	\begin{minipage}[t]{0.32\columnwidth}
		\centering
        \includegraphics[width=1\linewidth]{ProtoNet+CL.pdf}
        \subcaption{ProtoNet+CL}
		\label{fig:supp_visual_protonet_cl}
	\end{minipage}
	\begin{minipage}[t]{0.32\columnwidth}
		\centering
        \includegraphics[width=1\linewidth]{ProtoNet+Ours.pdf}
        \subcaption{ProtoNet+Ours}
		\label{fig:supp_visual_protonet_ours}
	\end{minipage}
    \\
    \begin{minipage}[t]{0.32\columnwidth}
		\centering
        \includegraphics[width=1\linewidth]{baseline.pdf}
        \subcaption{baseline}
		\label{fig:supp_visual_baseline}
	\end{minipage}
    \begin{minipage}[t]{0.32\columnwidth}
		\centering
        \includegraphics[width=1\linewidth]{baseline+CL.pdf}
        \subcaption{baseline+CL}
		\label{fig:supp_visual_baseline_cl}
	\end{minipage}
    \begin{minipage}[t]{0.32\columnwidth}
		\centering
        \includegraphics[width=1\linewidth]{Ours.pdf}
        \subcaption{Ours}
		\label{fig:supp_visual_ours}
	\end{minipage}
\caption{Visualization of 100 randomly sampled images for each of the 5 meta-test classes from miniImageNet by t-SNE.}
\label{fig:supp_visual_experiment}
\end{figure}


\vspace{-40pt}

\begin{table}[!ht]
\centering
\caption{Quantitative analysis of feature embeddings using SVM.}
\label{tab:svm_results}
\resizebox{0.4\columnwidth}{!}{%
\begin{tabular}{l|c}
\hline
Method        & Mean accuracy \\ \hline
ProtoNet      & 0.87          \\
ProtoNet+Ours & 0.91          \\
baseline      & 0.89          \\
Ours          & \textbf{0.98} \\ \hline
\end{tabular}%
}
\end{table}


We further give quantitative analysis below.
We use the same sampling strategy as in the visualization experiments above and divide the training and test sets in a 1:4 ratio.
Then the features extracted by the four methods ProtoNet, ProtoNet+Ours, baseline and Ours are classified with SVM.
The mean accuracies of these methods are shown in \tablename~\ref{tab:svm_results}.
The results indicate that the two-stage methods combined with our framework make feature embeddings more separable.

